PAC-learning in the presence of evasion adversaries

The existence of evasion attacks during the test phase of machine learning algorithms represents a significant challenge to both their deployment and understanding. These attacks can be carried out by adding imperceptible perturbations to inputs to generate adversarial examples and finding effective defenses and detectors has proven to be difficult. In this paper, we step away from the attack-defense arms race and seek to understand the limits of what can be learned in the presence of an evasion adversary. In particular, we extend the Probably Approximately Correct (PAC)-learning framework to account for the presence of an adversary. We first define corrupted hypothesis classes which arise from standard binary hypothesis classes in the presence of an evasion adversary and derive the Vapnik-Chervonenkis (VC)-dimension for these, denoted as the adversarial VC-dimension. We then show that sample complexity upper bounds from the Fundamental Theorem of Statistical learning can be extended to the case of evasion adversaries, where the sample complexity is controlled by the adversarial VC-dimension. We then explicitly derive the adversarial VC-dimension for halfspace classifiers in the presence of a sample-wise norm-constrained adversary of the type commonly studied for evasion attacks and show that it is the same as the standard VC-dimension, closing an open question. Finally, we prove that the adversarial VC-dimension can be either larger or smaller than the standard VC-dimension depending on the hypothesis class and adversary, making it an interesting object of study in its own right.

==> convex.tex <==
\section{Analyzing halfspace classifiers}
Let the standard 0-1 loss defined on the space $\mathcal{Y} \times \mathbb{R} \rightarrow \{0,1\}$ be $\ell(y,s)$, where $y$ is a label and $s$ is the real-valued score output by the halfspace classifier $\V{w}^T\V{x}+b$. If we assume that the space of labels is $\{-1,1\}$, then the 0-1 loss is defined as
\begin{align*}
    \ell(y,s) = \frac{\text{sign}(-ys)+1}{2}.
\end{align*}
From the idea of degraded classifiers discussed in Section \ref{subsec:degraded}, it is clear that whenever the output $\bot$ is obtained, the classifier is wrong and thus adds to the loss. In order to account for this in the loss function directly, we modify the loss function such that there is a non-zero loss when the output score is less than a certain threshold. For halfspace classifiers, the score is a direct measure of the distance from the classification boundary, so we add a constant to the initial loss such that the loss is only zero if the classification outcome is correct \emph{and} the score is higher than that constant. Without loss of generality, we set the constant to be equal to 1, so the modified loss function $\ell'(y,s)$ is
\begin{align*}
    \ell'(y,s) = \frac{\text{sign}(-ys+1)+1}{2}.
\end{align*}

Now, if the constraint \cite{goodfellow2014explaining} on the adversary is of the form $\bm{\delta} \in C$, where $C$ is a convex set, then the constraint we have to impose on the halfspace learning problem is $\V{w}^T \bm{\delta} \leq 1$. Otherwise, we will violate the degraded hypothesis formulation.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

